SEDAT:Security Enhanced Device Attestation with TPM2.0

Remote attestation is one of the ways to verify the state of an untrusted device. Earlier research has attempted remote verification of a devices' state using hardware, software, or hybrid approaches. Majority of them have used Attestation Key as a hardware root of trust, which does not detect hardware modification or counterfeit issues. In addition, they do not have a secure communication channel between verifier and prover, which makes them susceptible to modern security attacks. This paper presents SEDAT, a novel methodology for remote attestation of the device via a security enhanced communication channel. SEDAT performs hardware, firmware, and software attestation. SEDAT enhances the communication protocol security between verifier and prover by using the Single Packet Authorization (SPA) technique, which provides replay and Denial of Service (DoS) protection. SEDAT provides a way for verifier to get on-demand device integrity and authenticity status via a secure channel. It also enables the verifier to detect counterfeit hardware, change in firmware, and software code on the device. SEDAT validates the manufacturers` root CA certificate, platform certificate, endorsement certificate (EK), and attributes certificates to perform platform hardware attestation. SEDAT is the first known tool that represents firmware, and Integrity Measurement Authority (IMA) event logs in the Canonical Event Logs (CEL) format (recommended by Trusted Computing Group). SEDAT is the first implementation, to the best of our knowledge, that showcases end to end hardware, firmware, and software remote attestation using Trusted Platform Module (TPM2.0) which is resilient to DoS and replay attacks. SEDAT is the first remote verifier that is capable of retrieving a TPM2.0 quote from prover and validate it after regeneration, using a software TPM2.0 quote check.

==> assumptions.tex <==
\subsection{Assumptions and Limitations of SEDAT}  
\par SEDAT is implemented keeping hardware as root of trust using TPM2.0. All the devices provisioned with SEDAT requires to have hardware or firmware TPM2.0. Devices should have installed intel's latest TPM2-TSS, TPM2-abrmd and TPM2-tools. SEDAT assumes that, there is one time trusted secure channel for verifier to get all the root certificates from the device vendor. SEDAT uses single packet authorization for securing communication channel between prover and verifer. So, SEDAT assumes that pre-shared secret key is loaded at both ends before communication start between varifier and prover. It is protected from replay and DoS attacks but covering some advance attacks are out of scope of this research. All prover devices are required to be patched with provided IMA and firmware patches and latest linux kernel to get firmware and IMA event logs in CEL format. Protecting the prover or verifier from physical, side channel attacks is out of scope. SEDAT can be validated on Software TPM with intels TPM2 stack.    


==> goals.tex <==
{\bf {Goals and Contributions:}}

\par To the best of our knowledge, SEDAT is first proof of concept work for remote attestation and verifier to ensure the integrity and authenticity of devices via a security-enhanced communication channel.
\begin{itemize}
\item {\bf{Client provisioning}:} Provide tool for client provisioning. it is the process which enables platform owner to register the device with remote verifier using security enhanced SPA technique.
  \item {\bf{Platform attestation}:} Provide remote verifier for platform which attests platform root CA certificates, endorsement certificates, platform bindings.
  \item {\bf{CEL firmware eventlog}:} Provide tools to convert and verify firmware event logs into canonical event log (CEL) structure. also, validated upstremed kernel patches for crypto align firmware event logs.
\item {\bf{CEL IMA eventlogs}:} Provide tools and kernel patches for getting IMA eventlogs into userspace and converting it into CEL format.
\item {\bf{Quote check}:} Provide tools to check the quote at remote verifier.
\item {\bf{Secure authentication}:} Provide tools for secure connection and authentication for verifier and protects it from replay and DoS type attacks. 
\end{itemize}
 
\par This is not correct at this time --putting some placeholder flow. outline We review in Section 2 existing attestation protocols,
relevant adversary models and DoS attacks on attestation. In Sec
tion 3, we provide required preliminaries and notations, identify
the minimal requirements for secure non-interactive attestation
and describe SEDAT. Two prototype implementation of SEDAT are
then described in Section 4, its application to collective attestation
is explained in Section 5, and performance results are shown in Sec-
tion 6. Next, security of SEDAT is evaluated in Section 7. Related work
is summarized in Section 8 and the paper concludes in Section 9.

==> limitations.tex <==
\section{Limitations of Current Solutions}   
\par In recent research papers and in practice tpm has been used for hardware root of trust and remote attestation. where the integrity and authenticity of platform is relied on tpm based attestation key (AIK or AK). 
\begin{itemize}

\item {\bf{AK limitation}:}
\par AK is taken as hardware root of trust anchor for remote attestation. problem in that is, generation of AK comes few step later in device manufacturing process. AK is derived from endorsement key (EK) and EK is provided from platform/hardware vendor by fusing private key and exposing associated public key as explained in section above. So, AK based attestation fails to detect malicious or counterfiet hardware (in supply chain menufacturing process) as there is no validation for authenticity and integrity of hardware platform, the TPM module or both, if they are tempered, counterfieted or malicious. if both TPM module and platform (hardware device on which tpm is placed) are genuein but the binding that platform A should have hardware TPM module A is not verified, then also EK certificate and generated platform certificate will be different. in such cases, malicious hardware counterfitting is not detected by the remote attestation tool and AK is generated using malicious hardware's EK.
\item {\bf{Firmware eventlogs limitation}:}
\par Firmware components measurements, extension into pcr and execution is logged into firmware memory in form of firmware event logs.so, if the verifier validates firmware event logs, it will suffice the requirement of firmware validation. however, the problem with current state of firmware eventlogs is that, they are not crypto aliened format and not avaliable in user space. They are only available in UEFI shell. So, it needs to be read from ACPI table to user space. second problem is it does not have sequence number for the events. so, its hard to read the events and keep track of them from the binary blob when transfered to remote verifier. 
\item {\bf{Software eventlogs limitation}:}
\par Same as firmware event logs, IMA event logs also does not have sequence numbers so it is hard to keep track of it when sent on the remote verifier. second major problem is, since it is stored into small firmware memory which is not ment for storing incremental large IMA event logs.it needs the mechanisum to free up the space once the blob is read in user space.
\item {\bf{Quote check limitation}:}
\par In some of the attestation techniques, they have implemeted quote generation with nonce and checks it at the provers end only. as quote is non reversible operation.
\item {\bf{Protection to known attacks}:}
\par Some of the available solution and attestation protocols have tried to enchance the security against replay and DoS attacks but majority of the attestation framework takes the https protocol as secure communication channel which leave a place for malicious prover to flood the verifier, delay it or spoof the traffic to redirect and mislead.   
\end{itemize}

\par This limitations motivated our research to create remote verfier which can overcome all or majority of the above issues. So, lets discuss the requirements of the remote verifier first and then explain details about SEDAT. 


